ASCENT: A Context-Aware Spectrum Coexistence Design and Implementation Toolset for Policymakers in Satellite Bands

This paper introduces ASCENT (context Aware Spectrum Coexistence Design and Implementation) toolset, an advanced context-aware terrestrial satellite spectrum sharing toolset designed for researchers, policymakers, and regulators. It serves two essential purposes (a) evaluating the potential for harmful interference to primary users in satellite bands and (b) facilitating the analysis, design, and implementation of diverse regulatory policies on spectrum usage and sharing. Notably, ASCENT implements a closed-loop feedback system that allows dynamic adaptation of policies according to a wide range of contextual factors (e.g., weather, buildings, summer/winter foliage, etc.) and feedback on the impact of these policies through realistic simulation. Specifically, ASCENT comprises the following components (i) interference evaluation tool for evaluating interference at the incumbents in a spectrum-sharing environment while taking the underlying contexts, (ii) dynamic spectrum access (DSA) framework for providing context-aware instructions to adapt networking parameters and control secondary terrestrial network's access to the shared spectrum band according to context aware prioritization, (iii) Context broker to acquire essential and relevant contexts from external context information providers; and (iv) DSA Database to store dynamic and static contexts and the regulator's policy information. The closed-loop feedback system of ASCENT is implemented by integrating these components in a modular software architecture. A case study of sharing the lower 12 GHz Ku band (12.2-12.7 GHz) with the 5G terrestrial cellular network is considered, and the usability of ASCENT is demonstrated by dynamically changing exclusion zone's radius in different weather conditions.

==> Sections/Sections_I.tex <==
\vspace{-0.5cm}
\section{The Current State of 12 GHz Spectrum Sharing}
%This section summarizes the current spectrum sharing policy of the United States in 12 GHz band, and highlights the conflicts among different interest groups in sharing the 12 GHz band with the terrestrial 5G networks.

%\subsection{Present Spectrum Sharing Policy in 12 GHz Band}
%The Federal Commission of Communications (FCC) allows 12 GHz spectrum sharing between the primary DBS and co-primary MVDDS operations, where a one-way digital fixed non-broadcast service, including one-way direct-to-home  wireless service is permitted for MVDDS licensees.  The FCC enforces strict co-existence rules, such as frequency coordination, maximum effective isotropic radiated power (EIRP), and transmitter locations, on MVDDS licensees to ensure that MVDDS operations do not cause harmful interference with DBS receivers. 
%In particular, the existing policy limits the effective isotropic radiated power (EIRP) for MVDDS stations to 14.0 dBm per 24 MHz bandwidth. 
%Furthermore, prior to beginning operations, the MVDDS licensees must  ensure that the equivalent power flux density (EPFD) from a proposed transmitting antenna does not exceed the applicable EPFD limit at any DBS subscriber location. 
%In this context, the MVDDS licensees must conduct an initial survey of the area to determine the location of the DBS customers and remediate all complaints of interference. Thereafter, the burden shifts to the DBS licensees for new customers to take into account the presence of the MVDDS licensee and must remediate all complaints of interference. 
%Meanwhile, NGSO FSS  and MVDDS licensees share the 12 GHz band on a co-primary basis. These two services are given priority over one another in the shared band on the basis of first to deploy.
%%Currently, there are existing NGSO FSS currently deployed and using the band. However, MVDDS licensees have not successfully deployed systems that are currently using the band. Therefore the impact of the MVDDS systems is still speculative.

%\vspace{-0.2cm}
%\subsection{Summary of the Positions of the Stakeholders}

%In 2017, the federal commission of communications (FCC) conditioned access on the 12 GHz band on the outcome of a 2016 Petition for rulemaking, requesting that the unused NGSO FSS allocation on the 12.2-12.7 GHz band be deleted or demoted to secondary status. The petition also requested to allow MVDDs to provide two-way, point-to-point or mobile broadband services on the band. Around the same time, the MVDDS 5G Coalition released two coexistence studies demonstrating the new rules would protect DBS operators on the band but would be incompatible with NGSO FSS provider \cite{Peters_2016}. At the same time, the WorldVu Satellites Limited (OneWeb) also planned for a low-earth orbit NGSO satellite system in the 10.7–12.7 GHz band.  Weighing both initiatives, the FCC concluded that the reforms from the MVDDS 5G Coalition’s petition was not a sufficient reason to delay or deny the NGSO requests to use the 12 GHz band. However, the FCC did condition access to the 12 GHz band on the outcome of the petition and any other rulemaking reform or petitions from the FCC. Since these initial reforms, the FCC has been focused on releasing spectrum for 5G use on multiple bands beyond the 12 GHz spectrum. For instance, in 2020, the FCC initiated a proceeding to consider rule changes allowing the provision of 5G backhaul and broadband to ships and aircrafts in motion on additional bands. Overall, 5G has been priority for the FCC in establishing the spectrum sharing rules while taking the  ``highest-and-best use'' of the spectrum into consideration


%The existing policy allows for more established delineation of responsibility in sharing band between the MVDDS licensees and DBS providers. However, the sharing requirements and responsibilities between the MVDDS licensees and NGSO providers is still very ambiguous. This becomes further complicated by deploying 5G  services over the 12 GHz band. Specifically, NGSO providers are already using the band and have invested substantially toward developing their services on the band. Essentially, there has been contention from both sides of that facet of the spectrum sharing issue – can the two services coexist on the band? If they can, what parameters are necessary to ensure access and quality control for both services? If they cannot, which service should take precedence? Finally, what implications would a decision one way or another have on future regulation regarding spectrum sharing? We emphasize that different stakeholders posses different points-of-view on these issues, making 12 GHz band sharing between 5G and the existing wireless services a nationwide controversial issue. 

%In an attempt to establish best use for the band, the FCC released a Notice of Proposed Rulemaking (NPRM) in 2021 seeking comments on the feasibility and technical approach of deploying 5G services in 12 GHz band while protecting the incumbent operations in the band from harmful interference \cite{FCC}. 
%Specifically, the FCC is considering reevaluating the existing policy in order to put the 12 GHz band to its highest-value and most efficient use in the public interest. 
%Since the release of the NPRM, several interest groups submitted divergent comments to the FCC. MVDDS licensees strongly recommend that terrestrial 5G networks can co-exist in the 12 GHz band without any or with little coordination. They cite small cell sizes and advanced multi-antenna beam-forming technology as potential solutions. In contrast, both NGSO FSS and DBS licensees contend that terrestrial 5G networks can not be operated in the 12 GHz band without causing severe interference to their existing operations.  An overview of the analyses conducted by the major incumbent licensees of the 12 GHz band is briefly summarized in Table I. Due to the conflicting opinions and evidence presented, sharing the 12 GHz band with the proposed terrestrial 5G networks has become a highly controversial issue.  In the process of analyzing the filings from both 5G interests and incumbent parties, the authors neither take a stand on the accuracy of the analysis or veracity of the assertions from any given party.


%More specifically, the MVDDS licensees strongly advocate for allowing the two-way mobile communications and fixed services in the 12 GHz band  by updating the current spectrum sharing rules. Such an standpoint is heavily influenced by  the recent study demonstrating that the 5G cellular operations can coexist in the 12 GHz band without causing harmful interference at the NGSO FSS receivers \cite {RKF}. Furthermore, expanding the use of MVDDS on 12 GHz band  would encourage competition by delivering more choices and lower costs for consumers, thus prioritizing the terrestrial services as the ``highest and best use'' for the 12 GHz band. In contrast to the aforesaid claims of the MVDDS licensees, NGSO service providers contend that the 5G deployments in 12 GHz band would result in harmful interference at FSS user terminals and cause serious service disruptions \cite{Space_X}.  In fact, the standpoint of the NGSO service providers is that the NGSO licensees have the existing and established commercial and public service initiatives in place, making NGSO services as the ``highest and best use'' of the 12 GHz band.  Meanwhile, the DBS licensees have also raised concerns about the potential  deleterious impact of 5G deployment on 12 GHz band on the existing  DBS services. A recent study from DirectTV claims that the terrestrial mobile operations could potentially generate harmful interference at the DBS receivers, resulting packet loss, frozen video, and cancelled subscriptions \cite{Direct_TV}. However, the fellow DBS provider, DISH network, has confronted the study of DIRECTV due to the unrealistic assumptions on the 5G operations and DBS receivers \cite{DISH}. Overall, there are several discrepancies among the viewpoints of the major incumbent licensees regarding the feasibility of the deploying 5G cellular networks in the 12 GHz band.  

The Federal Communications Commission (FCC) allows 12 GHz spectrum sharing between the primary DBS and co-primary MVDDS operations, where a one-way digital fixed non-broadcast service, including one-way direct-to-home wireless service, is permitted for MVDDS licensees. MVDDS licensees must comply with strict coexistence rules, including frequency coordination, maximum effective isotropic radiated power (EIRP), and transmitter locations, to avoid harmful interference with DBS receivers. Meanwhile, NGSO FSS and MVDDS licensees share the 12 GHz band on a co-primary basis. Based on which service is deployed first, these two have priority over one another.

In 2021, the FCC released a Notice of Proposed Rulemaking (NPRM) seeking comments on whether 5G services could be deployed in the 12 GHz band while protecting incumbents from harmful interference \cite{FCC}. Since the release of the NPRM, several interest groups submitted divergent comments to the FCC. MVDDS licensees strongly recommend that terrestrial 5G networks can co-exist in the 12 GHz band without any or with little coordination. They cite small cell sizes and advanced multi-antenna beam-forming technology as potential solutions. In contrast, both NGSO FSS and DBS licensees contend that terrestrial 5G networks cannot be operated in the 12 GHz band without causing severe interference to their existing operations. An overview of the analyses conducted by the major incumbent licensees of the 12 GHz band is briefly summarized in Table I. The authors do not take a position on the accuracy of the analysis or the veracity of the assertions made by any parties.


 
    \setlength{\textfloatsep}{0pt}
	\begin{table*}
	\renewcommand{\arraystretch}{1.1}
	\small
	\centering
	\caption{\textcolor{black}{Comparison of Industry Specific Assertions on 12 GHz Spectrum Sharing with Terrestrial 5G Networks}}
	\label{table_0}
	\begin{tabularx}{\textwidth}{|l|X|X|X|}
	    \hline
Industry    & Overview of the Assertion & Key Features of the Assertion  & Criticism of the Assertion \\
	\hline
    MVDDS \cite{RKF} &\vspace{-0.2cm} \begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{Coexistence scenario:} Spectrum sharing between terrestrial 5G and NGSO FSS networks 
    
    \item 	\textbf{Key Point:} 5G can coexist with NGSO FSS receivers without interfering with them in $99.85\%$ cases
    
    \end{itemize}
    & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	\item Simulation setup for terrestrial 5G using macro and small cells and point-to-point wireless backhaul links for the continental USA
	
	\item 	Advanced antenna system at 5G BSs with sidelobe suppression
	\end{enumerate}  & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	
	\item 	Lack of realistic line-of-sight (LOS)  and  non-LOS (NLOS) propagation channel models
	
	\item Inaccurate assumptions about the deployment and characteristics of the FSS receivers \cite{Space_X}
	\end{enumerate}\\
	\hline
     NGSO FSS \cite{Space_X} & \vspace{-0.2cm} \begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{Coexistence scenario:} Spectrum sharing between  terrestrial 5G and NGSO FSS  networks
    
    \item 	\textbf{Key Point:} 5G operations in the 12 GHz band can disrupt NGSO FSS receivers, leading to $77\%$ service degradation
    
    \end{itemize}  & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	\item Accurate  modeling of the deployments of FSS receivers
	
	\item 	Practical antenna gain models for FSS receivers
	
	\item Non-probabilistic modeling of the LOS and NLOS propagation channels and FSS specific clutter loss models
	\end{enumerate}  & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	 \item A non-representative coexistence scenario of terrestrial 5G and NGSO FSS networks in the context of most of USA

	
	\item Unrealistic assumptions about the distribution of FSS receivers and 5G BSs, as outlined by proponents of 5G in the 12 GHz spectrum  \cite{RKF_Reply}
	
%	\item Ignoring the existing capability of avoiding interference with the proposed 5G mobile services by operating the NGSO FSS links outside the 12.2-12.7 GHz band 
	\end{enumerate}\\
	\hline
	DBS \cite{Direct_TV} &  \vspace{-0.2cm} \begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{Coexistence scenario:} Spectrum sharing between  terrestrial 5G and DBS  networks
    
    \item 	\textbf{Key Point:} 5G operations in 12 GHz band can generate 20-30 dB more interference levels than the limit set by the FCC
    \end{itemize}
    & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	\item  Practical antenna gain model for DBS receivers
	\item  Advanced beam forming antenna array at 5G BSs with sidelobe suppression 
	\item Practical clutter loss models for roof mounted DBS receivers in urban, sub-urban, and rural scenarios
	\end{enumerate}  & \vspace{-0.2cm}\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	\item 	Excessive high density of macro BSs, representing a highly conservative coexistence scenario, as mentioned by proponents of 5G in the 12 GHz spectrum
	\item Consideration of $10$ times larger transmit power from the macro BSs than the nominal values  \cite{DISH}
	\end{enumerate}\\
	\hline
	\end{tabularx}
\end{table*}


%The concluding remarks of the submitted comments are divided into two mutually conflicting categories: (1) the terrestrial 5G networks can co-exist in the 12 GHz band without any or with little coordination and (2) the terrestrial 5G networks can not be operated in 12 GHz band without causing severe interference to the incumbent operations. 







 



